NeuriCam: Key-Frame Video Super-Resolution and Colorization for IoT Cameras

We present NeuriCam, a novel deep learning-based system to achieve video capture from low-power dual-mode IoT camera systems. Our idea is to design a dual-mode camera system where the first mode is low-power (1.1 mW) but only outputs grey-scale, low resolution, and noisy video and the second mode consumes much higher power (100 mW) but outputs color and higher resolution images. To reduce total energy consumption, we heavily duty cycle the high power mode to output an image only once every second. The data for this camera system is then wirelessly sent to a nearby plugged-in gateway, where we run our real-time neural network decoder to reconstruct a higher-resolution color video. To achieve this, we introduce an attention feature filter mechanism that assigns different weights to different features, based on the correlation between the feature map and the contents of the input frame at each spatial location. We design a wireless hardware prototype using off-the-shelf cameras and address practical issues including packet loss and perspective mismatch. Our evaluations show that our dual-camera approach reduces energy consumption by 7x compared to existing systems. Further, our model achieves an average greyscale PSNR gain of 3.7 dB over prior single and dual-camera video super-resolution methods and 5.6 dB RGB gain over prior color propagation methods. Open-source code: https://github.com/vb000/NeuriCam.

==> abstract.tex <==
\begin{abstract}


Video streaming is an extremely power-hungry application of low-power wireless cameras. Super-resolution is a promising solution for this application; however, in its canonical form, it requires the model to extract high-frequency details that may be non-existent in the input. In this work, we study an alternate formulation of this problem where we upscale a very low-resolution grayscale video using high-resolution color frames sparsely sampled in time, as ground-truth priors. Intuitively, the periodic key frames can allow us to produce more faithful reconstruction of high-resolution video as well as generalize the problem to color. Motivated by this, we present a deep learning method for key-frame based video super resolution and colorization. Our results show that the key frame-based approach can produce better details (1.5dB gain) compared to state-of-the-art super resolution networks, while consuming less than half the bandwidth and reducing on-device system power consumption by 6-30x over existing wireless cameras.
\end{abstract}

==> intro-1.tex <==
\section{Introduction}

The power consumption of video camera systems is a bottleneck  for multiple applications like security cameras~\cite{sachin1, starfish, batteryvideo1,batteryvideo2}, wearable cameras (e.g., Google glass),  robotics and sensor deployments  for wildlife monitoring and smart farms~\cite{wilds,chandra2021smart}. While advances in sensor hardware have enabled microphones, temperature and pressure sensors that are low-power (10 to 100 uW)~\cite{ekhonet,powifi},  camera sensor hardware can generate significantly more data and thus have   orders of magnitude higher power consumption~\cite{locamera-spec,hicamera-spec}. 


There is roughly a 100x difference in the power consumption of grey-scale, noisy, low resolution image sensors and higher resolution RGB sensors (Fig.~\ref{fig:power_graph}) --- the HM01B0 sensor supports grey-scale, noisy QQVGA (160x120) resolution and  consumes only 1.1~mW, while the OV7735 color sensor consumes 100~mW at VGA (640x480) resolution~\cite{locamera-spec,hicamera-spec}. Three key factors  contribute to this power difference.
\squishlist
\item {\it Video resolution.} In contrast to  a temperature sensor that outputs a single value, a VGA camera  outputs 640×480 pixels per frame. At a  frame rate of 15 fps, this is around 4.6 million pixels per second. Thus, increasing the video resolution requires both a higher clock rate and significantly more energy consumption   to support the I/O operations~\cite{videoio,powerscaling}.
\item {\it Supporting color.} RGB image sensors that can support color require  increasing the number of channels per pixel which further increases the clock rate and I/O requirements.
\item {\it Noise and dynamic range.}  CMOS image sensors can reduce the power consumption at the cost of a higher read noise and  fixed pattern noise. This however results in a lower signal to noise ratio (SNR) and dynamic range~\cite{Liu_cmosimage,cmosnoise}. 
\squishend



%As a result, prior work on low-power wireless video systems have been limited to greyscale and low-resolution video~\cite{xxx,xxx,xxx}. 



\begin{figure}[!t]
\centering
%\vskip -0.4 in
    \includegraphics[width=1\linewidth]{Plots/System_figure_neuricam.png}
     \vskip -0.2 in
    \caption{{\bf NeuriCam system.} Our dual mode IoT camera system captures  low-resolution  gray-scale video from a low-power camera and  reconstructs
    high-resolution color frames using the heavily duty cycled  high-resolution key-frames. The real-time neural network runs at the edge  router that is not power constrained.}
    \label{fig:fig1}
   \vskip -0.2in
\end{figure}



This paper  explores the following problem: can we design high resolution  color video camera systems while minimizing  camera energy  consumption? Our idea is to design a  dual-mode camera system where  the first mode is low power (1.1~mW) but only outputs grey-scale, low resolution and noisy video and the second mode consumes much higher power (100~mW) but outputs color and higher resolution images. To reduce total energy consumption, we heavily duty cycle the high  power camera to output an image only once every second. This data can  then be wirelessly streamed to a nearby plugged-in access point or router that is not power constrained, where we run our real-time   neural network decoder to reconstruct a higher resolution color video. 



Our dual-mode\footnote{Ideally, one could  design a custom camera IC that can   read out low resolution gray scale continuously and provide a higher resolution color frame periodically with minimal switching delay. In practice, given the switching delays and resolutions of commodity low-power cameras, we implement the dual-modes using two different cameras. In the rest of the paper, we reuse dual-mode and dual-camera interchangeable, given this context.} approach to low-power video capture has three key advantages. First, heavily duty cycling the high power image sensor reduces its energy consumption. For example, duty-cycling it to capture one frame per second, can reduce its average power consumption  by a factor of the target frame rate (e.g., a power reduction of roughly 15x for 15 fps video). Second, capturing lower resolution monochrome video for the remaining frames, can significantly reduce the amount of data captured by the camera system. For example, capturing greyscale 160x120 video at 15 fps and the key frame instead of RGB 640x480 video reduces the amount of data captured by a factor of 48. Finally, the router can combine the data across the two streams by super-resolving the low-resolution grey-scale video using the heavily duty-cycled  high-resolution video frames, which we refer to as key-frames. We show that these  key-frames  act as ground-truth priors for reconstructing precise high-frequency details that is missing in the low-resolution frames. In addition, these key-frames are also a  source of information for color, allowing us to generalize the super-resolution task to color. 


\begin{figure}
    \centering
    \vskip 0.05in
    \includegraphics[width=\linewidth]{Plots/power_graph_1.pdf}
    \vskip -0.15in
    \caption{{Power v/s resolution  of commercially available low-power image sensors.} While the list is not exhaustive, it shows the general relationship between power and resolution.}
    \label{fig:power_graph}
    \vskip -0.15in
\end{figure}





%Video streaming has traditionally been considered an extremely power-hungry operation.  
%It is challenging to obtain high-quality video data from low-power  wireless devices across a range of applications from battery-powered and battery-free security cameras~\cite{batteryvideo1,batteryvideo2}, wearable cameras (e.g., Google glasses) as well as untethered and insect-scale  robots~\cite{sciencerobotics_uw,sciencerobotics_eu}.

Reconstructing high resolution color video from our low-power dual-camera system is challenging for three reasons: (i) since the input video from the always-ON camera is grey-scale, key frames from the heavily duty-cycled color camera are the only source of color. One na\"ive approach is to use the closest key frame to propagate color across the video. However, occlusions in the current frame may not always be present in the closest key frame due to motion, (ii) since we  capture the  higher resolution color key frames only once per second, there can be significant relative motion between the objects in the key frame and current frame.  Standard convolutional  operations mostly focus on local features and if there is a significant relative motion between these frames, they tend to fail to capture features that may have moved hundreds of pixels away, and (iii)  since in our practical implementation, we use two cameras in slightly different locations, we can not assume that the transformation between the two views will preserve parallel lines. Thus, we need to account for a change in the perspective between the two cameras as well as   different fields of view while combining the data.


We present a novel deep learning-based system to achieve  video capture from low-power dual-mode IoT  systems. To achieve this, we tackle   key-frame based video super-resolution and colorization as a single problem. Our design uses a bidirectional recurrent network architecture that propagates information between the key-frames. The bidirectional nature of our network ensures that the two high-resolution key frames that appear before and after the low-resolution frames are both used to super-resolve and colorize the video. We introduce a novel attention feature filter mechanism that assigns different weights to different features, based on the
correlation between the feature map and contents of the input frame at {each spatial location}. This ensures that correct features are used across the two key-frames to colorize different objects in the current frames (see~\xref{section:attention}). To address the problem of high mobility across frames, we use optical flow based alignment as an initial step to do long range motion alignment, and then refine it using deformable convolutions. We also aggregate temporal information to extract  details from neighboring frames  using grid propagation (see~\xref{sec:details}). Finally, we use a  fixed homographic transformation method to match the perspective of the  low-resolution camera to that of the high-resolution camera and use these perspective-matched frames as input to our model (\xref{sec:practical}).

{\bf Benchmark evaluation.} We first evaluate our neural network using standard datasets to emulate a dual-mode system with different resolutions, which we train using the Vimeo-90K  dataset and perform evaluation on the Vid4, UDM10 and REDS4 datasets. The REDS4 dataset is a first-person point-of-view camera dataset with a lot of random motion. Our evaluation shows that:
\squishlist
\item Compared to state-of-the-art video super resolution techniques (BasicVSR++~\cite{chan2021basicvsr}), our key-frame based approach increases the grey-scale video PSNR by 1.7-4~dB across the three datasets.\footnote{For fairness, our PSNR computations exclude the key-frames.} These improvements in the video quality can help with more faithful reconstruction of finer details such as signs, letters, shapes and textures (Fig.~\ref{fig:vsr_qual_comp}) and are possible because we can learn from the finer details in the high-resolution key frames that are absence in the low-resolution video.
\item We achieve a 4-6~dB gain in the colorization performance compared to  prior color propagation methods (DEVC~\cite{10.1145/3197517.3201365}). In comparison to reference based image super resolution methods (TTSR~\cite{inproceedings}), our bidirectional recurrent method with attention mechanism that use the key-frames achieves a 4-7~dB performance improvement across the three datasets.
\squishend




\begin{table*}[t!]
\caption{{\bf Comparison of existing wireless video streaming systems.} Note that we  report active power when the system is  ON and streaming. \cite{batteryvideo1} uses analog backscatter where the SNR of each pixel significantly reduces with distance due to the analog nature of its proposed communication system. *Owing to our dual-mode design where the high resolution camera is heavily duty cycled, only 5.8~mW of this power is from our cameras (13x reduction), realizing our goal of making the camera sensor power negligible. The rest is consumed by the microcontrollers and radios, which we do not currently optimize in our system.}

\begin{center}
\vskip -0.15in
 \begin{tabular}{lccccc}
 \toprule
 & Active Power  & Resolution & Frame rate & Color & Comms\\ \hline
 BackCam~\cite{sachin1} & 9.7~mW & $160 \times  120$ & 1 fps & greyscale & backscatter\\
 BeetleCam~\cite{sciencerobotics_uw} &4.4-18 mW  & $160 \times  120$ & 1-5 fps & greyscale & radio \\
  WISPCam~\cite{wispcam} & 6~mW & $176 \times  144$ & 0.001 fps & greyscale & backscatter \\
  Video Backscatter~\cite{batteryvideo1} & \splitr{2.4~mW\\
 - (sim)} 
  & \splitr{$112\times 112$\\
  1080p (sim)}
  & \splitr{13 fps\\ 10-60 fps} & \splitr{greyscale\\color} & \splitr{analog \\ backscatter} \\
%  Glimpse~\cite{glimpse} & 744~mW & $640 \times 480$ & 30 fps & color & X \\\hline
  Blink~\cite{blink_power} & 700-1800~mW & $640\times 480$/740p & 7.5-30 fps & color & radio  \\
  Our prototype & 106~mW* & $640 \times 480$ & 15 fps & color & radio \\
 \hline
\end{tabular}
\label{table:systable}
\end{center}
\vskip -0.2in
\end{table*}

{\bf Hardware evaluation.} We prototype a low-power dual-camera hardware using off-the-shelf components. Our prototype includes a Himax HM01B0 image sensor capturing greyscale video at 15~fps and QQVGA resolution  and  a OmniVision OV7692 color VGA sensor capturing key-frames once every second.  Our prototype design includes microcontrollers and wireless radios to support data transmission from these devices. Our evaluation with our prototype hardware shows that,
\squishlist
\item On the data collected from our dual-camera hardware, we achieve an average gain of 3.7~dB in the PSNR of greyscale video in comparison with BasicVSR++. In comparison to TTSR, we see an RGB performance gain of 5.6~dB.
\item The runtime of our model on a  Nvidia RTX
2080 Ti GPU is around 54 ms per frame. For context, at 15 fps, the receiver must process each frame in less than 66~ms to be real-time. By increasing the batch size and GPU utilization, we can reduce the per-frame processing time to 44~ms.
\item Our  system can achieve color 640x480 wireless video streaming at 15~fps while consuming only 46~mA. The active power is much lower than existing wireless video streaming systems at  comparable frame rates and resolution (Table.~\ref{table:systable}).
\squishend






\vskip 0.05in\noindent{\bf Contributions.} We address the problem of designing high resolution color video camera systems while minimizing camera energy consumption. To this end, 1)  we introduce a dual-mode camera approach where the first mode is low power but outputs grey-scale, low resolution video while the second mode is high power but outputs heavily duty-cycled color and higher resolution images. 2) we design an efficient deep learning technique for key-frame based video super resolution and colorization. 3) we address practical issues including perspective mismatch and wireless packet losses. 4) We provide extensive evaluations showing  significant gains over state-of-the-art video super resolution methods as well as prior color propagation methods. 5)  We built a prototype hardware that shows significant energy savings achieved by our low-power wireless camera system. 6) By making our algorithms and designs open-source at publication, we will help sustain progress in creating these low-power video systems. 

%At a high level, we model this problem by recurrent spatial warping of key-frames without explicit
%estimation of motion. The recurrent objective of the model is to predict a 
%high-resolution output frame, $ h_t $, given the low-resolution input frame, $l_t$, and
%the previous frame, $p_{t-1}$. Where, the previous frame, $p_{t-1}$, is used to
%incorporate the key-frames: $p_{t-1}$ is equal to the key-frame, $k_{t-1}$, when a key-frame
%corresponding to $l_{t-1}$ is available, else it is equal to the previous prediction
%$h_{t-1}$. We observed that, using last predicted frames and key-frames interchangeably
%allows us maintain the objective function constant regardless of the frequency of
%key-frames, resulting in better model performance. 



%Existing approaches to key frame-based video super-resolution  use traditional image processing techniques, achieve only a 2x quality improvement~\cite{xx,xx} and  do not support colorization. In contrast, we present the first deep learning technique for key frame-based video super-resolution. The use of neural networks instead of traditional image processing techniques allows us to achieve a 4x quality improvement. Furthermore, our technique works with low-quality gray-scale video and high-quality color key frames to produce high-quality colorized video. At a high level, we model this problem by recurrent spatial warping of key-frames without explicit
%estimation of motion. The recurrent objective of the model is to predict a 
%high-resolution output frame, $ h_t $, given the low-resolution input frame, $l_t$, and
%the previous frame, $p_{t-1}$. Where, the previous frame, $p_{t-1}$, is used to
%incorporate the key-frames: $p_{t-1}$ is equal to the key-frame, $k_{t-1}$, when a key-frame
%corresponding to $l_{t-1}$ is available, else it is equal to the previous prediction
%$h_{t-1}$. We observed that, using last predicted frames and key-frames interchangeably
%allows us maintain the objective function constant regardless of the frequency of
%key-frames, resulting in better model performance. 


%\begin{itemize}
%\item  We propose an efficient deep learning technique for key-frame based video super-resolution and colorization.
%\item We perform  experiments that show that, using a fraction of data-rate, our method produces significantly better quality output than state-of-the-art video super-resolution methods, showing the effectiveness of our method for low-power video streaming.
%\item We present a power analysis based on off-the-shelf hardware components showing that wireless cameras system based
% on our approach can reduce the on-device power consumption by 6-30x over existing wireless cameras.
%\end{itemize}






==> intro.tex <==
\section{Introduction}

%Video streaming has traditionally been considered an extremely power-hungry operation.  
%It is challenging to obtain high-quality video data from low-power  wireless devices across a range of applications from battery-powered and battery-free security cameras~\cite{batteryvideo1,batteryvideo2}, wearable cameras (e.g., Google glasses) as well as untethered and insect-scale  robots~\cite{sciencerobotics_uw,sciencerobotics_eu}.
Streaming high-quality video from low-power wireless devices across a range of applications from battery-powered and battery-free security cameras~\cite{batteryvideo1,batteryvideo2}, wearable cameras (e.g., Google glasses) as well as untethered and insect-scale  robots~\cite{sciencerobotics_uw,sciencerobotics_eu} is a challenging problem.
State-of-the-art low-power systems can only stream 190 x 120 monochrome video at 5-15 frames per second (fps) while consuming 15-30 mW \cite{sciencerobotics_uw, 10.1145/3302506.3310403}. Higher quality streaming is difficult due to the significantly larger data-rates involved that consume a much higher power. A popular solution is to employ dedicated codec hardware and compress the video stream to reduce the  transmission data rates. While this approach brings down the power required for communication to manageable levels, it comes at the  cost of increased power consumption for data processing. For instance, a codec based design results in the  system power consumption of around 1~W for streaming 720p video at 30 fps ~\cite{10.1145/3302506.3310403, 211271}. Thus, so far, there has been a strict tradeoff between wireless video quality and system power consumption.

This paper  explores the following problem: can we achieve high quality video streaming at low power? This requires us to minimize both the total data transmitted  as well as the amount of computation required for on-device video compression. A potential solution using pre-existing algorithms is to transmit low-quality video and use super-resolution to enhance the video quality at the receiver. While super-resolution can increase video quality, it is well known to be an ill-posed problem because of the intrinsic loss of information in a low-quality video due to non-invertible low-pass filtering and subsampling operations~\cite{Cands2012TowardsAM, 1033210}. This implies that, considering
information present in low-resolution inputs alone can result in many plausible output frames
for a given input frame.
%Furthermore, super-resolution is a  one-to-many mapping from the low-resolution to high-resolution video and determining the right solution is challenging. 


%To mitigate this inherent limitation of super-resolution, we ask what more information one can provide in the input to improve the output quality, while keeping the overall power consumption low? Taking

%To address this problem, we take inspiration from the concept of key-frames in 
%traditional video compression algorithms and
%propose a key-frame based super-resolution and colorization approach for
%low-power video streaming.

To address this problem,  we propose a key-frame based
super-resolution and colorization approach for low-power video streaming.
In this approach, we super-resolve a low-resolution grayscale 
video using sparsely sampled high-resolution video frames, 
referred to as key-frames. We show that the key-frames 
can act as ground-truth priors for reconstructing precise high-frequency
details. In addition to that, key-frames are also a great source of information
for color, allowing us to generalize the super-resolution task to color dimension.
This means that the low-resolution input to the model could just be a gray-scale video. While
some additional power is required for capturing key-frames it
can be offset with the power saved by capturing only gray-scale low-resolution
video instead of its color version. %This approach can be realized either with a multi-mode image sensor that can be switched between to low-resolution and high-resolution modes at run-time, or with a dual-camera system comprising of separate low-resolution and high-resolution sensors sharing a common perspective with the help of a beam-splitter \citep{vaezijoze2020imagepairs}.
Key-frame based super-resolution has not received much attention from the research community in
recent years, but several methods are proposed for this problem \cite{6205616, 4711756, 5604296}.
The methods propose motion compensated block matching methods to map
key-frames to low-resolution input frames. These methods only consider 2x scaling, while
we work with 4x scaling.
Furthermore, these methods do not consider the problem of colorization using
key-frames. To the best of our knowledge, this is the first deep learning technique
to tackle both key-frame based video super-resolution and colorization as a single problem.

%At a high level, we model this problem by recurrent spatial warping of key-frames without explicit
%estimation of motion. The recurrent objective of the model is to predict a 
%high-resolution output frame, $ h_t $, given the low-resolution input frame, $l_t$, and
%the previous frame, $p_{t-1}$. Where, the previous frame, $p_{t-1}$, is used to
%incorporate the key-frames: $p_{t-1}$ is equal to the key-frame, $k_{t-1}$, when a key-frame
%corresponding to $l_{t-1}$ is available, else it is equal to the previous prediction
%$h_{t-1}$. We observed that, using last predicted frames and key-frames interchangeably
%allows us maintain the objective function constant regardless of the frequency of
%key-frames, resulting in better model performance. 



%Existing approaches to key frame-based video super-resolution  use traditional image processing techniques, achieve only a 2x quality improvement~\cite{xx,xx} and  do not support colorization. In contrast, we present the first deep learning technique for key frame-based video super-resolution. The use of neural networks instead of traditional image processing techniques allows us to achieve a 4x quality improvement. Furthermore, our technique works with low-quality gray-scale video and high-quality color key frames to produce high-quality colorized video. At a high level, we model this problem by recurrent spatial warping of key-frames without explicit
%estimation of motion. The recurrent objective of the model is to predict a 
%high-resolution output frame, $ h_t $, given the low-resolution input frame, $l_t$, and
%the previous frame, $p_{t-1}$. Where, the previous frame, $p_{t-1}$, is used to
%incorporate the key-frames: $p_{t-1}$ is equal to the key-frame, $k_{t-1}$, when a key-frame
%corresponding to $l_{t-1}$ is available, else it is equal to the previous prediction
%$h_{t-1}$. We observed that, using last predicted frames and key-frames interchangeably
%allows us maintain the objective function constant regardless of the frequency of
%key-frames, resulting in better model performance. 

Our contributions in this work can be summarized as follows: (1) We propose an efficient deep learning technique for key-frame based
video super-resolution and colorization. (2) We perform  experiments that show that, using a fraction of data-rate, our method
produces significantly better quality output than state-of-the-art video
super-resolution methods. (3) We present a power analysis based on off-the-shelf hardware components showing that wireless cameras system based
on our approach can reduce the on-device power consumption by 6-30x over existing wireless cameras.

%\begin{itemize}
%\item  We propose an efficient deep learning technique for key-frame based video super-resolution and colorization.
%\item We perform  experiments that show that, using a fraction of data-rate, our method produces significantly better quality output than state-of-the-art video super-resolution methods, showing the effectiveness of our method for low-power video streaming.
%\item We present a power analysis based on off-the-shelf hardware components showing that wireless cameras system based
% on our approach can reduce the on-device power consumption by 6-30x over existing wireless cameras.
%\end{itemize}


\begin{figure}[!t]
\centering
\vskip -0.4 in
    \includegraphics[width=1\linewidth]{Plots/System_figure_neuricam.pdf}
     \vskip -0.2 in
    \caption{Overview of key-frame based super-resolution and colorization (KFSR).
    We use low-resolution  gray-scale frames and reconstruct
    high-resolution color frames using color inferred from the periodic high-resolution key-frames.}
    \label{fig:block}
    \vskip -0.18in
\end{figure}




==> related.tex <==
\section{Related Work}


\textbf{Video Super-resolution}. Super-resolution is a classic computer vision problem
that has gained renewed popularity with the effectiveness of deep learning methods
\cite{10.5555/2969239.2969266, 8099502, 8578791, 8237536, 7780576, 8099787}. Variations
to traditional convolution operation like sub-pixel convolutions \cite{7780576}, deformable
convolutions \cite{8237351, 8953797, tian2020tdan, 8237351, wang2019edvr} have been shown to
work well for video super-resolution. \cite{8578438} proposes generating dynamic filters 
\cite{10.5555/3157096.3157171} on the fly at run-time to generate sharp frames without
having to do explicit motion compensation. However, more recently, it has been shown that
recurrent networks \cite{RBPN2019, 10.1007/978-3-030-58610-2_38, chan2021basicvsr} can outperform 
feed-forward networks that operate on a small batch of frames, at much lower complexity. In contrast to this paper's use of high-resolution key-frames, these works and other recent prior work \cite{chan2021basicvsr, cvprw_2017_zhang_fast} perform super-resolution using low-resolution frames and hence cannot extract high-frequency details that may be non-existent in the low-resolution  input.

%\citep{chan2021basicvsr, cvprw_2017_zhang_fast}.  These works perform super-resolution on these low-resolution frames and the rest of the frames are super-resolved using motion information and residual present in the encoded bit stream referring to super-resolved key-frames. This however requires computing the motion information that is compute-intensive.  key-frames in the context of super-resolving a compressed video, where key-frames are super-resolved first and then the rest of the frames are super-resolved using motion information and residual present in the encoded bit stream referring to super-resolved key-frames. This however requires computing the motion information that is compute-intensive. The concept of key-frames is also used in the context of traditional super-resolution \citep{chan2021basicvsr, cvprw_2017_zhang_fast}. \citep{cvprw_2017_zhang_fast} uses key-frames in the context of super-resolving a compressed video, where key-frames are super-resolved first and then the rest of the frames are super-resolved using motion information and residual present in the encoded bit stream referring to super-resolved key-frames. \citep{chan2021basicvsr} denotes few of the low-resolution input frames as key-frames, and then uses the super-resolved versions of those to super-resolve other frames.

\textbf{Key-Frame based super-resolution}. Early work on key-frame based super-resolution
considers this problem as a special case of more general example-based super-resolution problem 
\cite{988747}, where a low-resolution image or video is super-resolved based on a pool of
high resolution images. While generalized block matching methods based on some distance
metric have been proposed for the example-based super-resolution problem \cite{988747, 6489325},
works on key-frame based super-resolution specialize those methods by performing
motion compensated block matching. Those methods, however, only achieve a 2x scaling  and do not consider color. Recent related work  on reference-based super-resolution (RefSR)
\cite{Zheng2017LearningCC, zheng2018crossnet, 9328132, 9157498, inproceedings} only consider images,  not video, and do not transfer color. 

\textbf{Video Colorization}. Early work on colorization focused on techniques to propagate user
edits or suggestions to other parts of an image using optimization techniques 
\cite{10.1145/1015706.1015780, 10.5555/2383847.2383887}. More recently, deep learning
methods have been shown to be more effective by gaining a higher level understanding of
image contents \cite{7410412, Endo2016DeepPropED, 10.1145/2897824.2925974,
8100206,10.1007/978-3-030-58610-2_38, zhang2017real}. These methods are primarily
designed for image editing applications, and need color hints at precise locations.
As a result, they tend to lose temporal coherence within a few frames \cite{Meyer18Color}.
One of the seminal works on video color propagation by Welsh et al. \cite{1693344},
suggesting that color spaces that separate luminance and color channels work better than
RGB color space. In recent years, many deep learning methods have been proposed for
color propagation problem to achieve reliable transfer of color for large number of
frames \cite{jampani:vpn:2017, 10.1007/978-3-319-46487-9_39, Meyer18Color}. These methods
operate on input videos in original resolution and as a result do not perform scaling
on luminance channel. In contrast, our method both scales the luminance channel and
propagates color.


{\bf Video compression.} Most commercial wireless cameras use on-device video compression algorithms to reduce the data transmission rate, including  recent work that uses neural networks for on-device video compression~\cite{wu2018vcii,Rippel2019LearnedVC,8953892}. These algorithms, however, are  designed for internet video streaming and more traditionally television broadcasting applications, which assumed a complex encoder running on a compute-intensive device and a simple decoder for the compute-constrained device side. Low-power wireless cameras on the other hand have reversed complexity, where the encoder is extremely resource constrained, but the decoder can be relatively complex. Our work explores the use of key-frame based super resolution for low-power video streaming.

%\textbf{Wireless Video Streaming}. \citep{745120} uses a combination of image compression on-device, and a simple pixel-difference based motion detection on the receiver to compress the input video and limit the data rate. \citep{726968} on the other hand doesn't use image compression but implements a remote control mechanism that can trigger the transmission of a single image. \citep{6142537, 7422694} propose low-power image compression techniques for wireless camera systems, and also serve as great references for limits on power consumption of compression-based techniques. \citep{1693344, 4415154} demonstrates wireless camera systems designed for medical diagnosis. For efficient transmission of video frames, \citep{10.1145/3302506.3310403, 211271} employs on-device averaging based motion detection algorithms to detect and transmit only image blocks that  have changed. More recently, \citep{211271, 8719264} have proposed back-scatter energy  harvesting systems for achieving battery-free wireless video streaming. These works demonstrate systems operating at low-resolutions and implementations only output gray scale frames. 

==> results.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\caption{Quantitative comparison on \textit{Vid4} dataset. Higher is better. Best results are in bold
and second best results are underlined. (RKFN = our work.)}
\label{comparison-vid4}
\centering
\begin{tabular}{@{}lcccccccc@{}}
\toprule
\multirow{2}{*}{} & \multicolumn{2}{c}{Calendar (Y)} & \multicolumn{2}{c}{City (Y)} & \multicolumn{2}{c}{Foliage (Y)} & \multicolumn{2}{c}{Walk (Y)} \\
 & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM \\
\midrule
TOFlow \cite{xue2019video} & 22.29 & 0.7273 & 26.79 & 0.7446 & 25.31 & 0.7118 & 29.02 & 0.8799 \\
FRVSR \cite{8578791} & 22.67 & 0.7844 & 27.70 & 0.8063 & 25.83 & 0.7541 & 29.72 & 0.8971 \\
DUF \cite{8578438} & 24.17 & 0.8161 & 28.05 & 0.8235 & 26.42 & 0.7758 & 30.91 & 0.9165 \\
RBPN \cite{RBPN2019} & 24.02 & 0.8088 & 27.83 & 0.8045 & 26.21 & 0.7579 & 30.62 & 0.9111 \\
EDVR \cite{wang2019edvr} & 24.05 & 0.8147 & 28.00 & 0.8122 & 26.34 & 0.7635 & 31.02 & 0.9152 \\
RSDN \cite{10.1007/978-3-030-58610-2_38} & 24.60 & 0.8355 & 29.20 & 0.8527 & 26.84 & 0.7931 & 31.04 & 0.9210 \\
\midrule
RKFN ($K=30$) & 26.70 & 0.8988 & 29.39 & 0.8909 & 29.09 & 0.8784 & 32.02 & 0.9415 \\
RKFN ($K=24$) & 26.69 & 0.8976 & 29.38 & 0.8993 & 29.58 & 0.8937 & 31.98 & 0.9407 \\
RKFN ($K=15$) & {\ul 27.36} & {\ul 0.9116} & \textbf{30.94} & {\ul 0.9202} & {\ul 30.50} & {\ul 0.9146} & {\ul 32.93} & {\ul 0.9530} \\
RKFN ($K=10$) & \textbf{27.61} & \textbf{0.9168} & {\ul 30.72} & \textbf{0.9228} & \textbf{30.74} & \textbf{0.9202} & \textbf{33.29} & \textbf{0.9568} \\
\bottomrule
 %& \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}
\end{tabular}
\vskip -0.15in
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
\caption{Comparison of our method with best performing super-resolution methods
on both Y and RGB metrics. Runtime is the average time consumed
for reconstructing a HD (1280x720) frame (* result from the paper for a similar setup).
Bandwidth is input data-rate required
for each method. All quality metrics are in PSNR/SSIM format.}
\footnotesize
\label{comparison-avg}
\centering
\begin{tabular}{@{}lccccc@{}}
\toprule
  & \multicolumn{1}{c}{RSDN} & \multicolumn{1}{c}{IconVSR} & \multicolumn{1}{c}{RKFN} & \multicolumn{1}{c}{RKFN} & \multicolumn{1}{c}{RKFN} \\
 & \multicolumn{1}{c}{\citep{10.1007/978-3-030-58610-2_38}} & \multicolumn{1}{c}{\citep{chan2021basicvsr}} & \multicolumn{1}{c}{($K=30$)} & \multicolumn{1}{c}{($K=24$)} & \multicolumn{1}{c}{($K=15$)} \\
\midrule
Parameters (M) & 6.18 & 8.70 & 4.49 & 4.49 & 4.49 \\
Runtime (ms) & 95 & 70* & 51 & 51 & 51 \\ % BasicVSR is observed to 131ms but their paper claims 70?!
Bandwidth (bpp) & 1.5000 & 1.5000 & \textbf{0.6727} & {\ul 0.6955} & 0.7968 \\
\midrule
Vid4 (Y) & 27.92/0.8505 & 28.04/0.8570 & 29.30/0.9024 & {\ul 29.41/0.9078} & \textbf{30.46/0.9254} \\
Vid4 (RGB) & 26.43/0.8349 & 26.63/0.8451 & 26.95/0.8775 & {\ul 27.08/0.8835} & \textbf{28.23/0.9047} \\
Xiph720p30 (Y) & 28.26/0.8086 & 28.79/0.8264 & 29.66/0.8261 & {\ul 30.30/0.8413} & \textbf{30.62/0.8488} \\
Xiph720p30 (RGB) & 26.64/0.7710 & 27.02/{\ul 0.7846} & 26.94/0.7662 & {\ul 27.51}/0.7839 & \textbf{27.84/0.7923} \\
Xiph720p (Y) & 28.40/0.8161 & 28.76/0.8281 & 30.51/0.8532 & {\ul 31.36/0.8700} & \textbf{31.72/0.8778} \\
Xiph720p (RGB) & 26.78/0.7787 & 27.00/0.7859 & 27.70/0.7953 & {\ul 28.46/0.8152} & \textbf{28.77/0.8241} \\
\bottomrule
\end{tabular}
\vskip -0.15in
\end{table}

==> system-0.tex <==

\begin{figure}
    \centering
     \includegraphics[width=1\linewidth]{Figures/fig2_3.png}
        \caption{Comparison of frame 64 in \textit{mobcal} sequence of
        \textit{Xiph} dataset. Key-frame based super-resolution can generate
        more accurate details than canonical super-resolution methods. Full sized-picture
        on the left is original frame. From left to right, snippets are in the order:
        ground-truth, IconVSR \cite{chan2021basicvsr},
        RSDN \cite{10.1007/978-3-030-58610-2_38} and our work.}
    \label{fig:key_frame_sr}
    \vskip -0.08in
\end{figure}

\section{Method}


Key-frame based super-resolution can leverage
precise high-frequency information provided by key-frames, in addition to spatial and
temporal information in low-resolution frames. In the classic
super-resolution problem, it has been shown that
any number of low-resolution frames will not be able to provide high-frequency
information without considerable dis-ambiguity \cite{1033210}. The lack of exact
information in the input sequence means that the model has to assume a natural
prior for reconstructing high-frequency details. In contrast, key-frames based
super-resolution  has ground-truth reconstruction priors, specific to
each input, in the form of periodic key-frames. %In addition to serving as ground-truth reconstruction priors, key-frames can act as a source of color.

%With these two differences in the formulation of super-resolution problem, our experiments show that we can develop a very efficient low-power wireless video streaming system.


\subsection{Key-Frame based Super-Resolution and Colorization}
Recurrent models are shown to be very effective for super-resolution task \cite{8578791, 
10.1007/978-3-030-58610-2_38, chan2021basicvsr} because of their ability to remember
relatively long-term information compared to sliding window methods. Moreover,
\cite{10.1007/978-3-030-58610-2_38} shows that residual blocks are simple and powerful
building blocks for super-resolution. We propose Recurrent
Key-Frame Network (RKFN) for key-frame based super-resolution and colorization. We use
a recurrent element, called \textit{Frame Memory} as the building block for our network.
The exact architecture of the frame memory block we use is shown in the Figure \ref{fig:r}b.
Consider that $\{g_t\}_{t=0}^{t=N}$ is the set of N ground-truth frames
we want to reconstruct. With the downsampling and decolorization process 
modelled as $\mathcal{D}$, the set of input low-resolution gray-scale
frames $\{l_t\}_{t=0}^{t=N}$  can be written as, $\{l_t\}_{t=0}^{t=N} = \{\mathcal{D}(g_t)\}_{t=0}^{t=N}$.

Key-frames are sampled at a frequency determined by a run-time
parameter called the \textit{key-frame interval}. Key-frame interval
denoted by $K$, implies that every $K$th
ground-truth frame is sampled to obtain the set of key-frames. Further,
to save the bandwidth of a wireless streaming system based on this method,
key-frames can be encoded using a    low-power image compression method, $\mathcal{E}$.
To ensure that the size of key-frame set is equal to that of low-resolution
set, key-frames are sampled as:
\begin{equation}
\{k_t\}_{t=0}^{t=N} = \{\mathcal{E}(g_t)\}_{t=0}^{t=N} 
\cdot \{\textbf{1}\{t \equiv 0\ (\textrm{mod}\ K) \}_{t=0}^{t=N}\}
\end{equation}
The network operates in L*a*b* color space with inputs and outputs normalized
to [-1, 1] range. Since our formulation is a multi-modal problem requiring enhancements
in both resolution and color, we instantiate two separate frame memory blocks, one for L*
channel, and another for a* and b* channels. Let $\mathcal{F}_{k, L^*}$ and
$\mathcal{F}_{k, a^*b^*}$ be frame memories corresponding to L* channel
and a*b* channels, respectively. Then at time step $t$, the model estimates the
high-resolution frame $h_t$ and the hidden state $s_t$, using the previous output and
previous hidden state:
\begin{equation}
\begin{split}
    h_{t, L^*}, s_{t, L^*} &=
    \begin{cases} 
      \mathcal{F}_{k, L^*} (l_t, h_{t-1, L^*}, s_{t-1, L^*}) & k_t = 0 \\
      k_{t, L^*}, 0 & k_t \neq 0
    \end{cases} \\
    h_{t, a^*b^*}, s_{t, a^*b^*} &=
    \begin{cases} 
      \mathcal{F}_{k, a^*b^*} (l_t, h_{t-1, a^*b^*}, s_{t-1, a^*b^*}) & k_t = 0 \\
      k_{t, a^*b^*}, 0 & k_t \neq 0
    \end{cases}
\end{split}
\end{equation}
While it's natural to assume that, considering both previous and the next
key-frame for super-resolving the current frame might perform better than
considering a single key-frame alone, we found that,
at large enough key-frame intervals, aggregating information from farther key-frame
results in diminishing returns. We observed that such a bidirectional approach, 
results in poorer performance due to the
degradation in information propagated from farther key-frame, in addition
to the computation overhead incurred for aggregating more information.
So, to make the effective use of information in key-frames, we implement a
nearest key-frame inference method, as depicted in the Fig~\ref{fig:r}a.
At inference step, $n$, this method
operates on a subset of the video containing a key-frame to key-frame sequence, 
$\{l_t\}_{t=nK}^{t=(n+1)K}$ and $\{k_t\}_{t=nK}^{t=(n+1)K}$, and performs inference
from both key-frames converging to the center, so each high-resolution frame is estimated from
its closest key-frame.  All layers except the
output layer use ReLU activation function, while the output layer uses $\tanh$ activation function to
generate normalized outputs. We train  using Charbonnier loss \cite{413553} with $\epsilon = 10^{-3}$, which has
a regularizing effect and avoids over smoothing of details.

==> system-1.tex <==
\section{System Design}
Video camera systems in the IoT context, typically involve a transmitter that is power constrained, and a receiver with a relatively high
power budget. As seen in Table \ref{table:systable}, low-power video streaming systems operating on the order of 10mW are only able
to stream QQVGA (160x120) grayscale video at 1-5fps. On the other hand, high-resolution color video streaming systems consume
700-1800mW for streaming VGA (640x480) to HD resolutions. 
We observe that the sensor power is significant at high-resolutions due to the 
large number of pixels being activated for each frame as well as the  I/O required to handle the data rates. To reduce the sensor power while
also preserving the  high-frequency details available in high-resolution frames, we propose a dual-camera system where
the first camera is low power camera capturing 15fps grayscale video at 160x120 resolution, operating at 1.1mW, and the second
high-resolution camera capturing 1fps color video at 640x480 resolution, operating at 100mW, pre-duty cycling. The two video streams transmitted
from this transmitter are then fed to a neural network decoder on the receiver to generate 15~fps color video at 640x480 resolution. We also note that the power numbers   in Table \ref{table:systable} includes the  image sensors as well as communication and on-device processing. While, we reduce the amount of data captured by the sensor, one can optimize the energy consumption of communication by using backscatter communication, like prior approaches. This however is not in  the scope of our paper.


In this section, we describe the design process of the neural network model that works with the proposed sensing method as well as address practical issues such as perspective mismatch and packet losses.  We then  provide a  description of the hardware prototype we designed to demonstrate our method. 


\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.6\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Plots/model.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{0.15\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Plots/model_blocks.pdf}
    \end{subfigure}
    \caption{Model architecture.}
    \label{fig:model}
\end{figure*}


\subsection{Design of the neural network model}

The neural network model running on the receiver has to upscale and colorize the input low-resolution video stream using
periodic high-resolution frames, referred to as \textit{key-frames}. This can be framed as key-frame based video
super-resolution and colorization task, and hence can leverage recent developments in video super-resolution and
colorization works. Recent video restoration methods can fundamentally be classified into two categories: sliding
window methods and recurrent methods. Sliding window methods consider a small group of neighboring frames along at
each step to output current frame. While, recurrent methods operate on only one frame, but propagate a
high-dimensional hidden state to next step. During training, recurrent methods involve a long backpropagation chain
from start frame to the end frame through the hidden state. As a result, recurrent methods are harder for training and
hyper-parameter tuning compared to sliding window methods. Sliding window methods, however, in addition to failing
to capture long range information, also involve redundant computation starting from input frames at each step.
As a result, recurrent methods have show to be more efficient \cite{8578791, 10.1007/978-3-030-58610-2_38,
chan2021basicvsr}. Moreover, \cite{Isobe2020RevisitingTM, 10.1007/978-3-030-58610-2_38} shows that residual
blocks are efficient and powerful building blocks for super resolution. Since real-time operation is a primary
requirement of video streaming application, we adopt a recurrent approach and use residual blocks core feature
extraction and propagation element in our model. Specific to key-frame based super-resolution and colorization,
we design the model addressing following challenges:
\squishlist
    \item Since key-frames are received only once every second, the model should be capable of mapping objects in
    the key-frames to 15 low-resolution frames in the presence of large relative motion. This is especially
    challenging if an object in the current low-resolution frame is occluded in the key-frame. To address this,
    we implement a bidirectional recurrent network that propagates information from previous and next key-frame, and use
    an attention mechanism to selectively choose forward or backward features from each region of the image.
    \item In videos with high relative motion between subsequent frames, hidden states computed based on previous
    frames might align poorly with current frame. Since the convolution operations tend to fail to effectively consider
    global correlations \cite{dosovitskiy2020vit, DBLP:journals/corr/abs-2110-02178}, it is hard for residual blocks to
    transform previous frame features to align with the current frame. \cite{tian2020tdan, wang2019edvr} proposes the
    use of deformable convolutions to mitigate this problem. \cite{chan2022basicvsrplusplus} further improves this by
    using optical flow based alignment in a grid propagation mechanism, which we use as feature propagation mechanism
    in our network.
    \item Since the low-resolution and high-resolution sensors are spatially shifted relative to each other, the images
    captured by low-resolution and high-resolution sensors would have a different perspectives. Since having a same
    perspective would be beneficial for alignment, we compute a fixed homographic transformation for low-resolution
    frame to transform into high-resolution frame and use the transformed frames as inputs to the model.
\squishend

Figure ?? (a) shows the complete architecture of our neural network model implementing those ideas. We split input
video sequence into key-frame to key-frame sequences before they are fed into the network. So, in each iteration,
the network operates 16 low-resolution frames, $\{l_{t}\}_{t=0}^{t=15}$, and two key-frames (previous and next),
$\{k_{t}\}_{t=0}^{t=1}$. Multiple key-frame to key-frame sequences can be stacked along the batch dimension to
increase the throughput of the network. We discuss in detail each component of the architecture in the subsections
below.

\subsubsection{Residual feature extractors}
Initially, both the low-resolution and high-resolution input sequences are fed into residual feature extraction blocks
shown in Figure ?? (b). We use 5 residual blocks for low-resolution feature extractor and 7 residual blocks for
key-frame feature extractor. The first two convolutional layers in the key-frame feature extractor subsample the input
spatially while increase the channel depth to generate key-frame feature that have same dimensions as low-resolution
features. We use separate feature extraction blocks with independent parameter sets for low-resolution
frames and key-frames. The feature extractors used for individual low-resolution frames, or individual key-frames,
is the same, however.

\subsubsection{Grid propagation with deformable alignment}
Aggregating temporal information is important for extracting details from neighboring and key-frames. But with
relative motion between frames, features extracted from neighboring frames would not aligned with current frame
for effective feature aggregation, if only traditional convolutional building blocks (such as Figure ?? (b)) are
used. Several optical flow based or deformable convolution based methods are proposed in the literature
\cite{RBPN2019, tian2020tdan, wang2019edvr} . We use grid propagation with deformable alignment proposed by
\cite{chan2022basicvsrplusplus} that uses a combination of these approaches: using optical flow based alignment
as an initial step before applying deformable convolution results in the best performance. Furthermore, it uses
grid propagation shown in Figure ?? (a) to achieve feature aggregation over the entire input sequence refined
over multiple levels. Each cell in the grid is shown in Figure ?? (c), contains an flow based deformable alignment
module and residual feature propagation module. It has to be noted that alignment and propagation module at each
level are different (with unique parameter sets), but same module is used across all time steps.

\begin{figure}
    \centering
    \begin{subfigure}[b]{\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Plots/attn_comp_0.png}
    \end{subfigure}
    \begin{subfigure}[b]{\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Plots/attn_comp_1.png}
    \end{subfigure}
    \begin{subfigure}[b]{\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Plots/attn_comp_2.png}
    \end{subfigure}
    \caption{Demonstration of the effectiveness of attention mechanism on a fast motion sample. Top and
    middle pictures show first and second key-frames, respectively. Bottom picture shows the prediction
    of frame 7 by our models with and without attention. Model with attention is able to infer details
    from second key-frame due to it's higher correlation, while the model without attention generates
    ambiguous color output.}
    \label{fig:attn_comp}
\end{figure}

\subsubsection{Attention feature filters}
Since our method is based on extracting and mapping high-resolution details and color from key-frames,
it is vulnerable to corner cases where an unseen object appears in between the key-frames, and key-frame closer
to the corresponding low-resolution, which is align with more would not have that object present. This results in
blurred and grayed out details as show in Figure ??. While alignment and propagation is effective in aggregating
feature from the entire sequence, those blocks do not explicitly consider the content of the frame and it's
correlation to features at each level. To solve this problem, we propose feature filter based on attention
mechanism \cite{Bahdanau2015NeuralMT}, that assign varying level of weightage to each filter level, based on the
correlation between the feature map and contents of the input frame at \emph{each spatial location}.

At any timestep $t \in {0, 15}$, let $w \times h$ be the resolution of the low-resolution inputs,
$l_t \in \mathbb{R}^{w \times h \times 1}$ be the low-resolution input frame,
$f_{l,t} \in \mathbb{R}^{w \times h \times 64}$ be aggregated features output by alignment
and propagation blocks at level $l$. Then features computed by the attention feature filter,
$\hat{f}_{t} \in \mathbb{R}^{w \times h \times 64}$, is given by:
\begin{equation} \label{eq1}
\hat{f}_{t} = \sum_{l=0}^3 f_{l,t} \odot A(f_{l,t}, l_t)
\end{equation}
where $ A(f_{l,t}, l_t) \in \mathbb{R}^{w \times h} $ is the attention between low-resolution input frame
and the feature map at level $t$ at \emph{each spatial location}. And, $\odot$ denotes the element wise multiplication
between the feature map and attention value computed for that feature map at that spatial location. Using simple
dot product attention function, attention score function for each spatial location $(i, j)$:
\begin{equation} \label{eq2}
A(f_{l,t}, l_t) ^ {i,j} = Softmax(f_{l,t}^{i,j} \cdot l_t^{i,j})
\end{equation}
Essentially, the summation in equation \ref{eq1} is a weighted average of correlation between feature map and
low-resolution input frame at each spatial location, over all propagation levels. The effect of attention is
demonstrated in figure \ref{fig:attn_comp}, where we can observe that occluded region is better predicted by the model
with attention using information from the second key-frame, inspite of the frame 7 being closer in time, to the
previous to the next. The model without attention is able to predict structure well from the low-resolution
input, but it has fails to prioritize second key-frame to infer correct color.

\subsubsection{Perspective correction}
Using different sensors for low-resolution and high-resolution streams inevitably results in differences in
file-of-view and perspective of captured video streams. Since alignment of feature between key-frames and
low-resolution is important, misalignment in input stream would adversely affect the model's performance.
However, the camera location with respect to each other are fixed, so any transformation between is would be
fixed transformation that can be applied as prepossessing step to the model's input. As the two cameras might
be capturing different planes, we cannot assume the transformation between them to be an affine transformation.
But assuming planar views of both cameras, we can estimate the homographic transformation of the two views.
Given four reference points in low-resolution frame and key-frame, we can transform arbitrary point $(x, y)$
in low-resolution plane to key-frame plane $(x_k, x_k)$, by:
\begin{equation}
    \begin{bmatrix}
    x_k \\
    y_k \\
    1
    \end{bmatrix}
    =
    \begin{bmatrix}
    h_{11} & h_{12} & h_{13} \\
    h_{21} & h_{22} & h_{23} \\
    h_{31} & h_{32} & 1
    \end{bmatrix}
    \begin{bmatrix}
    x \\
    y \\
    1
    \end{bmatrix}
\end{equation}

We estimate the homographic matrix capturing an image of a scene with four know reference points. We then identify
them in the low-resolution frame and key-frame frame. Using the points in low-resolution frame as the start, we find
a set of parameters that lands at end points found in key-frames using opencv's \texttt{getPerspectiveTransform} method.
The resulting transoformation matrix is then applied as prepossessing step to the input of the model.
